Measurement of the 2$\nu\beta\beta$ Decay Half-life of $^{130}$Te with CUORE

We measured two-neutrino double beta decay of $^{130}$Te using an exposure of 300.7 kg$\cdot$yr accumulated with the CUORE detector. Using a Bayesian analysis to fit simulated spectra to experimental data, it was possible to disentangle all the major background sources and precisely measure the two-neutrino contribution. The half-life is in agreement with past measurements with a strongly reduced uncertainty: $T^{2\nu}_{1/2} = 7.71^{+0.08}_{-0.06}\mathrm{(stat.)}^{+0.12}_{-0.15}\mathrm{(syst.)}\times10^{20}$ yr. This measurement is the most precise determination of the $^{130}$Te 2$\nu\beta\beta$ decay half-life to date.

==> wordcount.tex <==
\newpage
\section{word count}
\detailtexcount{00main}
\newpage
To estimate the word equivalent for figures use the figure’s aspect ratio (width / height). The estimate is [(150 / aspect ratio) + 20 words] for single-column figures, and [300 / (0.5 * aspect ratio)] + 40 words for double-column figures.

Fig1> 1.7496296296 aspect ratio
words: [300 / (0.5* ar)] + 40 =  383

Fig 2: 1.4689054726 ar
words = [150 / ar] + 20 = 122

Total figure: 505 words

The word equivalent for tables is 13 words plus 6.5 words per line for single-column tables. Double-column tables count as 26 words plus 13 words per line.
Table: 46 words

OLDTotal: 2850 (wcount) + 505 + 46 = 3401 / 3750 (349 words below limit)

New: 3184 (wcount) + 505 + 46 = 3735/3750 (15 words below)
